Reddit and the Fourth Estate: Exploring the magnitude and effects of media influence on community level moderation on Reddit

Most platforms, including Reddit, face a dilemma when applying interventions such as subreddit bans to toxic communities -- do they risk angering their user base by proactively enforcing stricter controls on discourse or do they defer interventions at the risk of eventually triggering negative media reactions which might impact their advertising revenue? In this paper, we analyze Reddit's previous administrative interventions to understand one aspect of this dilemma: the relationship between the media and administrative interventions. More specifically, we make two primary contributions. First, using a mediation analysis framework, we find evidence that Reddit's interventions for violating their content policy for toxic content occur because of media pressure. Second, using interrupted time series analysis, we show that media attention on communities with toxic content only increases the problematic behavior associated with that community (both within the community itself and across the platform). However, we find no significant difference in the impact of administrative interventions on subreddits with and without media pressure. Taken all together, this study provides evidence of a media-driven moderation strategy at Reddit and also suggests that such a strategy may not have a significantly different impact than a more proactive strategy.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> tex-files/background.tex <==
\section{Background}

\subsection{Why is moderation hard}

We can start of by describing the current moderation techniques and how they are not scalable. Moreover, we can describe how difficult it is to decide the rules and then decide whether content is adhering to rules or not. Finally, we can also describe how Reddit or other platforms have evolved from starting off with bastion of free speech and then slowly evolving their moderation and becoming ever so slightly more restrictive.

\subsection{Why would reddit be reactive}
We should come up with reasons for why reddit is reactive, however in the paper we will not be focusing on these reasons. These are just here as part of the setup.

\begin{enumerate}
    \item Lack of knowledge. \\
    Reddit is not aware of the subreddit or its violation
    \item Lack of clarity. \\
    Whether the subreddit has actually violated or not. 
    \item Fear of losing users. \\
    Banning the violating subreddit will result in loss of users.
\end{enumerate}

\subsection{User, Administration and Investors relationship with toxicity}
\textit{Monetization and moderation}
Deciding the rules and deciding the level of moderation is imperative to the monetization of a platform. There are two ways moderation and monetization of a platform are related, 1) moderation can influence the number of users there are on the site 2) low moderation can influence advertisers to not advertise or investors to not invest.


==> tex-files/conclusion.tex <==
\section{Conclusion}


==> tex-files/cost.tex <==
\section{Reddit administrative actions come loss}
Content moderation is seen a commodity rather than a necessity provided by the social media for its platform. It helps to maintain a welcoming and civil platform for new users to join. Moderation also creates a platform favourable for advertisers and investors. There are cases where \note{Cite YouTube apocalypse, sleeping giants, twitter (for inversters)} advertisers and investors withdrew their interest from a platform entirely because of the bad image of the platform due to inappropriate content and lack of content moderation. The lack of initiative in moderation from Reddit is apparent in how its content policy grew over the years, driven mainly by criticism from media and users. We hypothesize the delay or lack of urgency in performing administrative actions is caused by the cost of the interventions. In their work, et al. show how platforms profit greatly from toxicity and extremist ideologies. Following this pattern, we aim to measure the revenue these communities bring and the revenue lost from closing these communities. Establishing a high cost to administrative actions will enable us understand would enable us to understand the lack of moderation in newer platforms and the inconsistencies in Reddit’s moderation.

\subsection{Revenue Streams}
As a social media hosting user-generated content, platforms Reddit’s primary source of revenue is advertisement and then paid memberships. Advertisers can place their ad on Reddits sidebar or in the middle of feed. Being the 7th most popular website in the US Reddit sees a lot of traffic with 330 million monthly active users \note{cite}. Valued at \$6 billion with a revenue of \$226 million for 2021 \note{cite} Reddit’s ARPU (Average Revenue per User) is estimated to be around \$0.68. Compared to \$7 and \$9 ARPU of Facebook and Twitter Reddit’s is still growing its business model to catch up. Apart from advertising, a smaller part of Reddit’s revenue comes from selling in-site currency: \textit{Gold}, \textit{Silver} and \textit{Platinum} coins. Users can buy these coins and give them to submissions or comments as awards. Given these two revenue streams, in the next section we highlight how we design experiments to measure the cost of interventions.

\subsection{Methods}
In testing the cost of intervention, we break the analysis into two categories 1) \textbf{Before Intervention}: how much revenue/activity were the closed communities bringing and 2) \textbf{After Intervention}: how revenue was lost after closing the communities. In measuring the revenue brought by a closed community before their closure we measure three values: 1) total amount of activity on the particular community, 2) total amount of Reddit currency i.e. coins spent on the community and 3) the number of users brought to the platform by the community.  

\subsection{Method}
list of methods:

\textbf{How much revenue was being made:}
\begin{itemize}
    \item How many users came to reddit for this subreddit
    \item How much gold/reddit currency was distributed here.
    \item How much user activity was generated here daily \\
\end{itemize}

\textbf{How much revenue was lost:}
\begin{itemize}
    \item Qualitative analysis of migration (searching for other platforms names in these communities)
    \item Loss of number of users.
\end{itemize}

\note{talk about how generally moderations can be costly.}


Table:

\begin{center}
\begin{tabular}{ c | c |  c | c | c}
 & \textbf{Banned} & \textbf{Toxic} & \textbf{Control} & \textbf{All} \\
 \midrule
Activity 		& 150M	& XM	& YM 	& KM	\\
Gold	 		& 3.2K	& 2.6K	& 1.3K 	& 250K	\\
Gold per Community 	& 55	& 60	& 43 	& 49	\\
Incoming 		& 1M	& 550K	& 410K 	& -	\\
\end{tabular}
\end{center}

\note{literature review on user migration}
\note{List all the different platforms that users might have migrated to, search their names in all platforms and then look at their revenue}

